A powerful test for differentially expressed gene pathways via graph-informed structural equation modeling

A major task in genetic studies is to identify genes related to human diseases and traits to understand functional characteristics of genetic mutations and enhance patient diagnosis. Besides marginal analyses of individual genes, identification of gene pathways, i.e., a set of genes with known interactions that collectively contribute to specific biological functions, can provide more biologically meaningful results. Such gene pathway analysis can be formulated into a high-dimensional two-sample testing problem. Due to the typically limited sample size of gene expression datasets, most existing two-sample tests may have compromised powers because they ignore or only inefficiently incorporate the auxiliary pathway information on gene interactions. We propose T2-DAG, a Hotelling's $T^2$-type test for detecting differentially expressed gene pathways, which efficiently leverages the auxiliary pathway information on gene interactions through a linear structural equation model. We establish the asymptotic distribution of the test statistic under pertinent assumptions. Simulation studies under various scenarios show that T2-DAG outperforms several representative existing methods with well-controlled type-I error rates and substantially improved powers, even with incomplete or inaccurate pathway information or unadjusted confounding effects. We also illustrate the performance of T2-DAG in an application to detect differentially expressed KEGG pathways between different stages of lung cancer.

==> arxiv_main <==
\begin{thebibliography}{48}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[Am{\'e}ndola et~al.(2020)Am{\'e}ndola, Dettling, Drton, Onori, and
  Wu]{amendola2020structure}
C.~Am{\'e}ndola, P.~Dettling, M.~Drton, F.~Onori, and J.~Wu.
\newblock Structure learning for cyclic linear causal models.
\newblock In \emph{Conference on Uncertainty in Artificial Intelligence}, pages
  999--1008. PMLR, 2020.

\bibitem[Ashburner et~al.(2000)Ashburner, Ball, Blake, Botstein, Butler,
  Cherry, Davis, Dolinski, Dwight, Eppig, et~al.]{ashburner2000gene}
M.~Ashburner, C.~A. Ball, J.~A. Blake, D.~Botstein, H.~Butler, J.~M. Cherry,
  A.~P. Davis, K.~Dolinski, S.~S. Dwight, J.~T. Eppig, et~al.
\newblock Gene ontology: tool for the unification of biology.
\newblock \emph{Nature genetics}, 25\penalty0 (1):\penalty0 25--29, 2000.

\bibitem[Bai and Saranadasa(1996)]{bai1996}
Z.~Bai and H.~Saranadasa.
\newblock Effect of high dimension: by an example of a two sample problem.
\newblock \emph{Statistica Sinica}, pages 311--329, 1996.

\bibitem[Bonferroni(1936)]{bonferroni1936teoria}
C.~Bonferroni.
\newblock Teoria statistica delle classi e calcolo delle probabilita.
\newblock \emph{Pubblicazioni del R Istituto Superiore di Scienze Economiche e
  Commericiali di Firenze}, 8:\penalty0 3--62, 1936.

\bibitem[Bouveyron et~al.(2007)Bouveyron, Girard, and
  Schmid]{bouveyron2007high}
C.~Bouveyron, S.~Girard, and C.~Schmid.
\newblock High-dimensional discriminant analysis.
\newblock \emph{Communications in Statistics—Theory and Methods}, 36\penalty0
  (14):\penalty0 2607--2623, 2007.

\bibitem[Cai and Jiang(2014)]{cai2014revealing}
B.~Cai and X.~Jiang.
\newblock Revealing biological pathways implicated in lung cancer from tcga
  gene expression data using gene set enrichment analysis.
\newblock \emph{Cancer Informatics}, 13:\penalty0 CIN--S13882, 2014.

\bibitem[Cai et~al.(2019)Cai, Lin, Girard, Zhou, Yang, Ci, Zhou, Luo, Yao,
  Tang, et~al.]{cai2019}
L.~Cai, S.~Lin, L.~Girard, Y.~Zhou, L.~Yang, B.~Ci, Q.~Zhou, D.~Luo, B.~Yao,
  H.~Tang, et~al.
\newblock Lce: an open web portal to explore gene expression and clinical
  associations in lung cancer.
\newblock \emph{Oncogene}, 38\penalty0 (14):\penalty0 2551--2564, 2019.

\bibitem[Cai et~al.(2014)Cai, Liu, and Xia]{cai2014}
T.~T. Cai, W.~Liu, and Y.~Xia.
\newblock Two-sample test of high dimensional means under dependence.
\newblock \emph{Journal of the Royal Statistical Society: Series B (Statistical
  Methodology)}, 76\penalty0 (2):\penalty0 349--372, 2014.

\bibitem[Chang et~al.(2015)Chang, Lee, and Huang]{chang2015impact}
J.~T.-H. Chang, Y.~M. Lee, and R.~S. Huang.
\newblock The impact of the cancer genome atlas on lung cancer.
\newblock \emph{Translational Research}, 166\penalty0 (6):\penalty0 568--585,
  2015.

\bibitem[Chen et~al.(2011)Chen, Paul, Prentice, and Wang]{chen2011regularized}
L.~S. Chen, D.~Paul, R.~L. Prentice, and P.~Wang.
\newblock A regularized hotelling’s t 2 test for pathway analysis in
  proteomic studies.
\newblock \emph{Journal of the American Statistical Association}, 106\penalty0
  (496):\penalty0 1345--1360, 2011.

\bibitem[Chen and Qin(2010)]{chen2010}
S.~X. Chen and Y.-L. Qin.
\newblock A two-sample test for high-dimensional data with applications to
  gene-set testing.
\newblock \emph{The Annals of Statistics}, 38\penalty0 (2):\penalty0 808--835,
  2010.

\bibitem[Chun et~al.(2015)Chun, Zhang, and Zhao]{chun2015gene}
H.~Chun, X.~Zhang, and H.~Zhao.
\newblock Gene regulation network inference with joint sparse gaussian
  graphical models.
\newblock \emph{Journal of Computational and Graphical Statistics}, 24\penalty0
  (4):\penalty0 954--974, 2015.

\bibitem[Consortium(2019)]{gene2019gene}
G.~O. Consortium.
\newblock The gene ontology resource: 20 years and still going strong.
\newblock \emph{Nucleic acids research}, 47\penalty0 (D1):\penalty0 D330--D338,
  2019.

\bibitem[Dancik and Theodorescu(2014)]{dancik2014robust}
G.~M. Dancik and D.~Theodorescu.
\newblock Robust prognostic gene expression signatures in bladder cancer and
  lung adenocarcinoma depend on cell cycle related genes.
\newblock \emph{PloS one}, 9\penalty0 (1):\penalty0 e85249, 2014.

\bibitem[Fan et~al.(2019)Fan, Jang, Sun, and Zhou]{fan2019precision}
R.~Fan, B.~Jang, Y.~Sun, and S.~Zhou.
\newblock Precision matrix estimation with noisy and missing data.
\newblock In \emph{The 22nd International Conference on Artificial Intelligence
  and Statistics}, pages 2810--2819. PMLR, 2019.

\bibitem[Friedman et~al.(2008)Friedman, Hastie, and
  Tibshirani]{friedman2008sparse}
J.~Friedman, T.~Hastie, and R.~Tibshirani.
\newblock Sparse inverse covariance estimation with the graphical lasso.
\newblock \emph{Biostatistics}, 9\penalty0 (3):\penalty0 432--441, 2008.

\bibitem[Gregory et~al.(2015)Gregory, Carroll, Baladandayuthapani, and
  Lahiri]{gregory2015}
K.~B. Gregory, R.~J. Carroll, V.~Baladandayuthapani, and S.~N. Lahiri.
\newblock A two-sample test for equality of means in high dimension.
\newblock \emph{Journal of the American Statistical Association}, 110\penalty0
  (510):\penalty0 837--849, 2015.

\bibitem[Hotelling(1931)]{hotelling1931}
H.~Hotelling.
\newblock The generalization of student's ratio.
\newblock \emph{The Annals of Mathematical Statistics}, 2\penalty0
  (3):\penalty0 360--378, 1931.

\bibitem[Huang et~al.(2006)Huang, Liu, Pourahmadi, and
  Liu]{huang2006covariance}
J.~Z. Huang, N.~Liu, M.~Pourahmadi, and L.~Liu.
\newblock Covariance matrix selection and estimation via penalised normal
  likelihood.
\newblock \emph{Biometrika}, 93\penalty0 (1):\penalty0 85--98, 2006.

\bibitem[Jacob et~al.(2012)Jacob, Neuvial, and Dudoit]{jacob2012}
L.~Jacob, P.~Neuvial, and S.~Dudoit.
\newblock More power via graph-structured tests for differential expression of
  gene networks.
\newblock \emph{The Annals of Applied Statistics}, 6\penalty0 (2):\penalty0
  561--600, 2012.

\bibitem[Kanehisa and Goto(2000)]{kanehisa2000}
M.~Kanehisa and S.~Goto.
\newblock Kegg: kyoto encyclopedia of genes and genomes.
\newblock \emph{Nucleic acids research}, 28\penalty0 (1):\penalty0 27--30,
  2000.

\bibitem[Kanehisa et~al.(2019)Kanehisa, Sato, Furumichi, Morishima, and
  Tanabe]{kanehisa2019}
M.~Kanehisa, Y.~Sato, M.~Furumichi, K.~Morishima, and M.~Tanabe.
\newblock New approach for understanding genome variations in kegg.
\newblock \emph{Nucleic acids research}, 47\penalty0 (D1):\penalty0 D590--D595,
  2019.

\bibitem[Kong et~al.(2020)Kong, Yao, Bing, Guo, Huang, Huang, and
  Lai]{kong2020dynamical}
C.~Kong, Y.-X. Yao, Z.-T. Bing, B.-H. Guo, L.~Huang, Z.-G. Huang, and Y.-C.
  Lai.
\newblock Dynamical network analysis reveals key micrornas in progressive
  stages of lung cancer.
\newblock \emph{PLOS Computational Biology}, 16\penalty0 (5):\penalty0
  e1007793, 2020.

\bibitem[Krishnamoorthy and Menon(2013)]{krishnamoorthy2013matrix}
A.~Krishnamoorthy and D.~Menon.
\newblock Matrix inversion using cholesky decomposition.
\newblock In \emph{2013 signal processing: Algorithms, architectures,
  arrangements, and applications (SPA)}, pages 70--72. IEEE, 2013.

\bibitem[Kuismin et~al.(2017)Kuismin, Kemppainen, and
  Sillanp{\"a}{\"a}]{kuismin2017precision}
M.~Kuismin, J.~Kemppainen, and M.~Sillanp{\"a}{\"a}.
\newblock Precision matrix estimation with rope.
\newblock \emph{Journal of Computational and Graphical Statistics}, 26\penalty0
  (3):\penalty0 682--694, 2017.

\bibitem[Li et~al.(2012)Li, Chun, and Zhao]{li2012sparse}
B.~Li, H.~Chun, and H.~Zhao.
\newblock Sparse estimation of conditional graphical models with application to
  gene networks.
\newblock \emph{Journal of the American Statistical Association}, 107\penalty0
  (497):\penalty0 152--167, 2012.

\bibitem[Li et~al.(2020)Li, Aue, Paul, Peng, and Wang]{li2020adaptable}
H.~Li, A.~Aue, D.~Paul, J.~Peng, and P.~Wang.
\newblock An adaptable generalization of hotelling’s $ t^2$ test in high
  dimension.
\newblock \emph{The Annals of Statistics}, 48\penalty0 (3):\penalty0
  1815--1847, 2020.

\bibitem[Loh and B{\"u}hlmann(2014)]{loh2014high}
P.-L. Loh and P.~B{\"u}hlmann.
\newblock High-dimensional learning of linear causal networks via inverse
  covariance estimation.
\newblock \emph{The Journal of Machine Learning Research}, 15\penalty0
  (1):\penalty0 3065--3105, 2014.

\bibitem[Long et~al.(2019)Long, Liu, Zhou, Yu, Tian, and
  Bao]{long2019identification}
T.~Long, Z.~Liu, X.~Zhou, S.~Yu, H.~Tian, and Y.~Bao.
\newblock Identification of differentially expressed genes and enriched
  pathways in lung cancer using bioinformatics analysis.
\newblock \emph{Molecular medicine reports}, 19\penalty0 (3):\penalty0
  2029--2040, 2019.

\bibitem[Lopes et~al.(2011)Lopes, Jacob, and Wainwright]{lopes2011more}
M.~Lopes, L.~Jacob, and M.~J. Wainwright.
\newblock A more powerful two-sample test in high dimensions using random
  projection.
\newblock In \emph{Advances in Neural Information Processing Systems}, pages
  1206--1214, 2011.

\bibitem[Love et~al.(2014)Love, Huber, and Anders]{love2014moderated}
M.~I. Love, W.~Huber, and S.~Anders.
\newblock Moderated estimation of fold change and dispersion for rna-seq data
  with deseq2.
\newblock \emph{Genome biology}, 15\penalty0 (12):\penalty0 550, 2014.

\bibitem[Network et~al.(2014)]{cancer2014}
C.~G. A.~R. Network et~al.
\newblock Comprehensive molecular profiling of lung adenocarcinoma.
\newblock \emph{Nature}, 511\penalty0 (7511):\penalty0 543--550, 2014.

\bibitem[Nishimura(2001)]{biocarta}
D.~Nishimura.
\newblock Biocarta.
\newblock \emph{Biotech Software \& Internet Report}, 2\penalty0 (3):\penalty0
  117--120, 2001.
\newblock \doi{10.1089/152791601750294344}.
\newblock URL \url{https://doi.org/10.1089/152791601750294344}.

\bibitem[Peters and B{\"u}hlmann(2014)]{peters2014identifiability}
J.~Peters and P.~B{\"u}hlmann.
\newblock Identifiability of gaussian structural equation models with equal
  error variances.
\newblock \emph{Biometrika}, 101\penalty0 (1):\penalty0 219--228, 2014.

\bibitem[{Quantitative Biomeical Research Center}(2019)]{LCE}
{Quantitative Biomeical Research Center}.
\newblock {Lung Cancer Explorer}.
\newblock \url{http://lce.biohpc.swmed.edu/}, 2019.
\newblock Accessed: 2021-06-15.

\bibitem[Robinson et~al.(2010)Robinson, McCarthy, and Smyth]{robinson2010edger}
M.~D. Robinson, D.~J. McCarthy, and G.~K. Smyth.
\newblock edger: a bioconductor package for differential expression analysis of
  digital gene expression data.
\newblock \emph{Bioinformatics}, 26\penalty0 (1):\penalty0 139--140, 2010.

\bibitem[Shao et~al.(2010)Shao, Wang, and He]{shao2010}
W.~Shao, D.~Wang, and J.~He.
\newblock The role of gene expression profiling in early-stage non-small cell
  lung cancer.
\newblock \emph{Journal of thoracic disease}, 2\penalty0 (2):\penalty0 89,
  2010.

\bibitem[Shojaie and Michailidis(2009)]{shojaie2009analysis}
A.~Shojaie and G.~Michailidis.
\newblock Analysis of gene sets based on the underlying regulatory network.
\newblock \emph{Journal of Computational Biology}, 16\penalty0 (3):\penalty0
  407--426, 2009.

\bibitem[Shojaie and Michailidis(2010)]{shojaie2010network}
A.~Shojaie and G.~Michailidis.
\newblock Network enrichment analysis in complex experiments.
\newblock \emph{Statistical applications in genetics and molecular biology},
  9\penalty0 (1), 2010.

\bibitem[Srivastava and Du(2008)]{srivastava2008test}
M.~S. Srivastava and M.~Du.
\newblock A test for the mean vector with fewer observations than the
  dimension.
\newblock \emph{Journal of Multivariate Analysis}, 99\penalty0 (3):\penalty0
  386--402, 2008.

\bibitem[Srivastava and Kubokawa(2013)]{srivastava2013}
M.~S. Srivastava and T.~Kubokawa.
\newblock Tests for multivariate analysis of variance in high dimension under
  non-normality.
\newblock \emph{Journal of Multivariate Analysis}, 115:\penalty0 204--216,
  2013.

\bibitem[Tibshirani(1996)]{tibshirani1996regression}
R.~Tibshirani.
\newblock Regression shrinkage and selection via the lasso.
\newblock \emph{Journal of the Royal Statistical Society: Series B
  (Methodological)}, 58\penalty0 (1):\penalty0 267--288, 1996.

\bibitem[Venugopal et~al.(2019)Venugopal, Yeh, Kodeboyina, Lee, Sharma, Patel,
  and Sharma]{venugopal2019differences}
N.~Venugopal, J.~Yeh, S.~K. Kodeboyina, T.~J. Lee, S.~Sharma, N.~Patel, and
  A.~Sharma.
\newblock Differences in the early stage gene expression profiles of lung
  adenocarcinoma and lung squamous cell carcinoma.
\newblock \emph{Oncology Letters}, 18\penalty0 (6):\penalty0 6572--6582, 2019.
\newblock \doi{10.3892/ol.2019.11013}.

\bibitem[Weiss and Kingsley(2008)]{weiss2008}
G.~J. Weiss and C.~Kingsley.
\newblock Pathway targets to explore in the treatment of non-small cell lung
  cancer.
\newblock \emph{Journal of Thoracic Oncology}, 3\penalty0 (11):\penalty0
  1342--1352, 2008.

\bibitem[Wille et~al.(2004)Wille, Zimmermann, Vranov{\'a}, F{\"u}rholz, Laule,
  Bleuler, Hennig, Preli{\'c}, von Rohr, Thiele, et~al.]{wille2004sparse}
A.~Wille, P.~Zimmermann, E.~Vranov{\'a}, A.~F{\"u}rholz, O.~Laule, S.~Bleuler,
  L.~Hennig, A.~Preli{\'c}, P.~von Rohr, L.~Thiele, et~al.
\newblock Sparse graphical gaussian modeling of the isoprenoid gene network in
  arabidopsis thaliana.
\newblock \emph{Genome biology}, 5\penalty0 (11):\penalty0 R92, 2004.

\bibitem[Wu and Pourahmadi(2003)]{wu2003nonparametric}
W.~B. Wu and M.~Pourahmadi.
\newblock Nonparametric estimation of large covariance matrices of longitudinal
  data.
\newblock \emph{Biometrika}, 90\penalty0 (4):\penalty0 831--844, 2003.

\bibitem[Xu et~al.(2016)Xu, Lin, Wei, and Pan]{xu2016}
G.~Xu, L.~Lin, P.~Wei, and W.~Pan.
\newblock An adaptive two-sample test for high-dimensional means.
\newblock \emph{Biometrika}, 103\penalty0 (3):\penalty0 609--624, 2016.

\bibitem[Zhang and Zou(2014)]{zhang2014sparse}
T.~Zhang and H.~Zou.
\newblock Sparse precision matrix estimation via lasso penalized d-trace loss.
\newblock \emph{Biometrika}, 101\penalty0 (1):\penalty0 103--120, 2014.

\end{thebibliography}

